TS-SEP: Joint Diarization and Separation Conditioned on Estimated Speaker Embeddings

Since diarization and source separation of meeting data are closely related tasks, we here propose an approach to perform the two objectives jointly. It builds upon the target-speaker voice activity detection (TS-VAD) diarization approach, which assumes that initial speaker embeddings are available. We replace the final combined speaker activity estimation network of TS-VAD with a network that produces speaker activity estimates at a time-frequency resolution. Those act as masks for source extraction, either via masking or via beamforming. The technique can be applied both for single-channel and multi-channel input and, in both cases, achieves a new state-of-the-art word error rate (WER) on the LibriCSS meeting data recognition task. We further compute speaker-aware and speaker-agnostic WERs to isolate the contribution of diarization errors to the overall WER performance.

==> Makefile <==
SHELL=/bin/bash

main := main


help:
	cat Makefile

# arXiv: ../interspeech_mmm_arxiv

cmp:
	# Download the view.pdf from arXiv and verify that they are equal
	diffpdf ${main}.pdf view.pdf


clean_ieee:
	rm -rf ieee
	rm -rf ieee_arXiv

ieee: clean_ieee
	# rsync -Rr . $@/
	git clone . $@/
	# rm -rf $@/.git
	cd $@ && rm New_IEEEtran_how-to.tex guidelines.tex
	
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_1.log
	cd $@ && bibtex ${main}
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_2.log
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_3.log
	
	arxiv_latex_cleaner $@ --keep_bib
	# mv $@_arXiv $@_upload
	cp main.pdf $@_arXiv/
	echo "See $@_arXiv/ for prepared files"
	
	cd $@_arXiv && tar -czf $@.tar.gz *

	echo "You can now upload $@.tar.gz"

clean_arXiv:
	rm -rf arXiv
	rm -rf arXiv_arXiv
	rm -rf arXiv.tar.gz

arXiv: clean_arXiv
	rsync -Rr . $@/  # https://askubuntu.com/a/942355/750373
	# cp -r  . $@/  # Does not work, but rsync works
	rm -rf $@/.git

	cd $@ && rm New_IEEEtran_how-to.tex
	# cd $@ && rm download.png

	# https://arxiv.org/help/00README
	cd $@ && echo 'nohypertex' > 00README.XXX

	# Rarely nessesary
	cd arXiv && echo '${main}.tex toplevelfile' >> 00README.XXX
	
	# Force arXiv to use pdflatex
	# Prepend "\pdfoutput=1\n" to the main file
	cd $@ && sed -i '1s;^;\\pdfoutput=1\n;' ${main}.tex

	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_1.log
	cd $@ && bibtex ${main}
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_2.log
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_3.log
	
	# \includegraphics{PB2019.eps} produces error on arXiv
	# -> ! Package pdftex.def Error: File `PB2019.pdf' not found.
	# cd $@ && mv PB2019-eps-converted-to.pdf PB2019.pdf
	# python -c 'import os, glob;\
	# files=[(\
	#     e,\
	#     e.replace("-eps-converted-to.pdf", ".pdf"),\
	#     ) for e in glob.glob("arXiv/*-eps-converted-to.pdf")];\
	# assert files;\
	# [(\
	#     os.rename(old, new), \
	#     print("Renamed", old, "to", new)\
	# ) for old, new in files]'

	# cd $@ && rm $(main).{acn,acr,glg,glo,gls,bbl,alg}  # keep for arxiv
	cd $@ && rm ${main}.{aux,blg,log}
	# cd $@ && rm $(main).{ist,lof,lot,out,run.xml,toc}  # does not exist
	# cd $@ && rm $(main)-blx.bib  # does not exist

	# cd $@ && rm convBF.synctex.gz
	cd $@ && mv ${main}.pdf ..

	arxiv_latex_cleaner $@ --keep_bib  # https://github.com/google-research/arxiv-latex-cleaner

	tar -czf $@.tar.gz -C $@_arXiv .

	echo "You can now upload $@.tar.gz"


==> fig_overview.tex <==




==> table_vad.tex <==
\begin{table*}[th]
\centering
  \caption{...}
    
    
    \sisetup{round-precision=1,round-mode=places, table-format = 3.1}
    \setlength\tabcolsep{2.8pt} %
  \begin{tabular}{ l | S S S S S S | S }
    \toprule
    \textbf{System} & \multicolumn{6}{c|}{\textbf{Overlap ratio in \%}} & {\textbf{Average}} \\
    & {$0$S} & {$0$L} & {$10$} & {$20$} & {$30$} & {$40$} & \\
    \midrule
    Chen et al. \cite{Chen2020LibriCSS} & 11.9 & 9.7 & 13.6 & 15.0 & 19.9 & 21.9 & 15.983124889414524 \\
Raj et al. \cite{Raj2021Meeting} & 11.2 & 8.5 & 10.6 & 14.8 & 15.5 & 17.5 & 13.4 \\
    Chen et al. \cite{Chen2021CSSConformer} & 5.2 & \thl 4.0 & 5.8 & 6.8 & 9.0 & 10.0 & 7.119566411815651 \\
    Wang et al. \cite{Wang2021CSSSpectralMapping} & 5.4 & 5.0 & 4.8 & \thl 5.0 & \thl 6.6 & \thl 7.6 & \thl 5.850056340389075 \\
    \bottomrule
  \end{tabular}
\end{table*}
\begin{table*}[th]
\centering
  \caption{
    Inits
  }
  \begin{tabular}{ l | S S }
    \toprule
        \textbf{System} & \textbf{\acrshort{DER}} & \textbf{\acrshort{WER}} \\
        \midrule
        Human annotations (Oracle) && \\
        Spectral Clustering (SC) && \\
    \bottomrule
  \end{tabular}
  
  \caption{
    VAD
    Init: Orcale, channels 1, no extraction
    Should I verify, which parameter/options were nessesary?
    Should it be shown in a table? e.g. showing that the DER or WER is > 100.
    Probably drop this table, if only one option works, it is boring.
  }
  \begin{tabular}{ l | S S }
    \toprule
        \textbf{Mixup} & \textbf{\acrshort{DER}} & \textbf{\acrshort{WER}} \\
        \midrule
        $p=0$ &&\\
        $p=0.5$ &&\\
        $p=1$ &&\\
    \bottomrule
  \end{tabular}
\end{table*}
\begin{table*}[th]
\centering

  \caption{
    VAD
    Init: Orcale, multi channels, Mixup $p=0.5$
    Does masking work without the threshold (i.e. irrelevant performance drop)?
    Table is too large. Is this interesting enough for VAD?
    Repeat table for Separation.
    Remove segmentation column
  }


\begin{tabular}{cccccccccccc}
	\toprule
  \bf Output & \bf Init & \bf WPE & \multicolumn{3}{c}{\bf Segmentation} & \multicolumn{2}{c}{\bf Extraction} & \multicolumn{2}{c}{\bf DER} & \multicolumn{2}{c}{\bf WER} \\
  \multicolumn{3}{c}{} & E & D & T & BF & Mask & DEV & EVAL & DEV & EVAL \\
	\midrule
	T & SC     & \xmark & 81 & 161 & 0.6 & \xmark &              & 21.62              & 20.2               & 34.45              & 31.79              \\  %
	T & SC     & \xmark & 81 & 81  & 0.6 & \xmark &              & 8.35               & 7.67               & 25.0               & 23.83              \\  %
	\midrule
	T & Oracle & \xmark & 81 & 161 & 0.1 & \xmark & \cmark (0.1) & \color{gray} 37.25 & \color{gray} 33.93 & \color{gray} 45.67 & \color{gray} 43.1  \\  %
	T & SC     & \xmark & 81 & 161 & 0.1 & \xmark & \cmark (0.1) & 39.02              & 35.57              & 47.69              & 44.7               \\  %
	\cmidrule{8-11}
	T & Oracle & \xmark & 81 & 81  & 0.1 & \xmark & \cmark (0.1) & \color{gray} 16.78 & \color{gray} 15.11 & \color{gray} 32.02 & \color{gray} 30.89 \\  %
	T & SC     & \xmark & 81 & 81  & 0.1 & \xmark & \cmark (0.1) & 18.27              & 16.63              & 34.09              & 32.5               \\  %
	\cmidrule{8-11}
	T & Oracle & \xmark & 81 & 81  & 0.6 & \xmark & \cmark (0.1) & \color{gray} 6.61  & \color{gray} 6.18  & \color{gray} 21.7  & \color{gray} 21.95 \\  %
	T & SC     & \xmark & 81 & 81  & 0.6 & \xmark & \cmark (0.1) & 8.35               & 7.67               & 24.82              & 23.65              \\  %
	\cmidrule{8-11}
	T & Oracle & \xmark & 81 & 161 & 0.6 & \xmark & \cmark (0.1) & \color{gray} 20.68 & \color{gray} 18.72 & \color{gray} 28.85 & \color{gray} 27.72 \\  %
	T & SC     & \xmark & 81 & 161 & 0.6 & \xmark & \cmark (0.1) & 21.62              & 20.2               & 31.12              & 29.42              \\  %
	\midrule
	T & Oracle & \cmark & 81 & 161 & 0.6 & \cmark & \cmark (0.1) & \color{gray} 16.66 & \color{gray} 15.76 & \color{gray} 12.82 & \color{gray} 14.6  \\  %
	T & SC     & \cmark & 81 & 161 & 0.6 & \cmark & \cmark (0.1) & 19.6               & 17.37              & 17.08              & 16.77              \\  %
	T & SC     & \cmark & 81 & 81  & 0.6 & \cmark & \cmark (0.1) & 7.77               & 6.24               & 17.97              & 16.89              \\  %
	T & Oracle & \cmark & 81 & 81  & 0.6 & \cmark & \cmark (0.1) & \color{gray} 4.73  & \color{gray} 4.65  & \color{gray} 13.91 & \color{gray} 15.06 \\  %
	\bottomrule
\end{tabular}

  
  \begin{tabular}{ c c c c c c c | S S }
    \toprule
        \textbf{Init} & \textbf{WPE} & \multicolumn{3}{c}{\textbf{Segmentation}} & \multicolumn{2}{c|}{\textbf{Extract}} & \textbf{\acrshort{DER}} & \textbf{\acrshort{WER}} \\
        & & E & D & T & {BF} & {Mask.} &  &  \\
        \midrule
        Oracle &  & 81 & 161 & 0.6 & \xmark & \xmark & & \\  %
        SC &  & 81 & 161 & 0.6 & \xmark & \xmark & 20.34 & 31.79 \\  %
        Oracle &  & 81 & 81 & 0.6 & \xmark & \xmark & & \\  %
        SC &  & 81 & 81 & 0.6 & \xmark & \xmark & 7.73 & 23.83 \\  %
        Oracle &  & 81 & 81 & 0.1 & \xmark & \xmark & & \\  %
        SC &  & 81 & 81 & 0.1 & \xmark & \xmark & 16.79 & 32.91 \\  %
        \midrule
        Oracle & & 81 & 161 & 0.1 & \xmark &\cmark (0.1) & \color{gray} 34.26 & \color{gray} 43.1 \\  %
        SC & & 81 & 161 & 0.1 & \xmark &\cmark (0.1) & 35.92 & 44.7 \\  %
        \cmidrule{8-9}
        Oracle & & 81 & 81 & 0.1 & \xmark &\cmark (0.1) & \color{gray} 15.28 & \color{gray} 30.89 \\  %
        SC & & 81 & 81 & 0.1 & \xmark &\cmark (0.1) & 16.79 & 32.5 \\  %
        \cmidrule{8-9}
        Oracle & & 81 & 81 & 0.6 & \xmark &\cmark (0.1) & \color{gray} 6.22 & \color{gray} 21.95 \\  %
        SC & & 81 & 81 & 0.6 & \xmark &\cmark (0.1) & 7.73 & 23.65 \\  %
        \cmidrule{8-9}
        Oracle & & 81 & 161 & 0.6 & \xmark &\cmark (0.1) & \color{gray} 18.92 & \color{gray} 27.72 \\  %
        SC & & 81 & 161 & 0.6 & \xmark &\cmark (0.1) & 20.34 & 29.42 \\  %
        \midrule
        Oracle & \cmark & 81 & 161 & 0.6 & \cmark &\cmark (0.1) & \color{gray} 15.85 & \color{gray} 14.6 \\  %
        SC & \cmark & 81 & 161 & 0.6 & \cmark &\cmark (0.1) & 17.59 & 16.77 \\  %
        SC & \cmark & 81 & 81 & 0.6 & \cmark &\cmark (0.1) & 6.39 & 16.89 \\  %
        Oracle & \cmark & 81 & 81 & 0.6 & \cmark &\cmark (0.1) & \color{gray} 4.66 & \color{gray} 15.06 \\  %
    \bottomrule
  \end{tabular}
  
\end{table*}
\begin{table*}[th]
\centering

  \caption{
    Separation System
    E, D, T = 81, 160, 0.6
  }
  \begin{tabular}{ c c c c | S S }
    \toprule
        \textbf{Init} & \textbf{WPE} & \multicolumn{2}{c|}{\textbf{Extraction}} & \textbf{\acrshort{DER}} & \textbf{\acrshort{WER}} \\
        & & {BF} & {Masking} &  &  \\
        \midrule
        Oracle & \xmark & \xmark & \xmark & \color{gray} 13.5 & \color{gray} 23.02 \\  %
        SC & \xmark & \xmark & \xmark & 14.9 & 24.59 \\  %
        Oracle & \cmark & \xmark & \xmark & \color{gray} 13.34 & \color{gray} 22.76 \\  %
        SC & \cmark & \xmark & \xmark & \bf 14.69 & 24.24 \\  %
        SC & \cmark & \xmark & \cmark (0) & \bf 14.69 & 10.5 \\  %
        SC & \cmark & \cmark & \xmark & \bf 14.69 & 9.02 \\  %
        SC & \cmark & \cmark & \cmark (0.1) & \bf 14.69 & \bf 8.72 \\  %
        SC & \xmark & \cmark & \cmark (0.1) & 14.92 & 9.87 \\  %
        Oracle & \cmark & \cmark & \cmark (0.1) & \color{gray} 13.34 & \color{gray} 6.76 \\  %
    \bottomrule
  \end{tabular}
  
\end{table*}
\begin{table*}[th]
\centering

  \caption{
    Separation System: Segmentation
    Convert frames to seconds?
    Includes WPE
  }
  
\begin{tabular}{cccccccccccc}
	\toprule
  \bf Output & \bf Init & \bf WPE & \multicolumn{3}{c}{\bf Segmentation} & \multicolumn{2}{c}{\bf Extraction} & \multicolumn{2}{c}{\bf DER} & \multicolumn{2}{c}{\bf WER} \\
  \multicolumn{3}{c}{} & E & D & T & BF & Mask & DEV & EVAL & DEV & EVAL \\
	\midrule
	T  & SC & \cmark & 81  & 81  & 0.6 & \cmark & \cmark (0.1) & 7.77  & 6.24  & 17.97 & 16.89 \\  %
	\midrule
	TF & SC & \cmark & 81  & 161 & 0.6 & \cmark & \cmark (0.1) & 16.48 & 14.49 & 10.69 & 8.72  \\  %
	TF & SC & \cmark & 81  & 141 & 0.6 & \cmark & \cmark (0.1) & 13.3  & 11.6  & 11.04 & 9.07  \\  %
	TF & SC & \cmark & 81  & 121 & 0.6 & \cmark & \cmark (0.1) & 10.45 & 9.13  & 11.45 & 9.64  \\  %
	TF & SC & \cmark & 81  & 101 & 0.6 & \cmark & \cmark (0.1) & 8.57  & 7.79  & 12.77 & 10.83 \\  %
	TF & SC & \cmark & 81  & 81  & 0.6 & \cmark & \cmark (0.1) & 9.45  & 8.94  & 17.23 & 15.51 \\  %
	\midrule
	TF & SC & \cmark & 81  & 81  & 0.3 & \cmark & \cmark (0.1) & 6.64  & 5.26  & 13.53 & 11.37 \\  %
	TF & SC & \cmark & 81  & 81  & 0.6 & \cmark & \cmark (0.1) & 9.45  & 8.94  & 17.23 & 15.51 \\  %
	TF & SC & \cmark & 81  & 81  & 0.3 & \cmark & \cmark (0.1) & 6.64  & 5.26  & 13.53 & 11.37 \\  %
	TF & SC & \cmark & 81  & 81  & 0.1 & \cmark & \cmark (0.1) & 6.96  & 5.27  & 12.04 & 9.84  \\  %
	\midrule
	TF & SC & \cmark & 101 & 101 & 0.6 & \cmark & \cmark (0.1) & 8.99  & 8.32  & 16.87 & 14.99 \\  %
	TF & SC & \cmark & 101 & 101 & 0.3 & \cmark & \cmark (0.1) & 6.78  & 5.19  & 13.52 & 11.33 \\  %
	TF & SC & \cmark & 101 & 101 & 0.1 & \cmark & \cmark (0.1) & 7.26  & 5.32  & 12.05 & 9.83  \\  %
	\midrule
	TF & SC & \cmark & 81  & 161 & 0.6 & \cmark & \cmark (0.1) & 16.48 & 14.49 & 10.69 & 8.72  \\  %
	TF & SC & \cmark & 81  & 161 & 0.3 & \cmark & \cmark (0.1) & 18.51 & 16.03 & 10.3  & 8.05  \\  %
	TF & SC & \cmark & 81  & 161 & 0.1 & \cmark & \cmark (0.1) & 20.94 & 18.36 & 10.46 & 8.25  \\  %
	\bottomrule
\end{tabular}

  
  \begin{tabular}{c c c c c c | S S }
    \toprule
        Output & \multicolumn{3}{c}{\textbf{Segmentation}} & \multicolumn{2}{c|}{\textbf{Extraction}} & \textbf{\acrshort{DER}} & \textbf{\acrshort{WER}} \\
        & Erosion & Dilation & Thresh. & BF & Mask. & & \\
        \midrule
        T & 101 & 101 & 0.6 & \xmark & \xmark & & \\
        T & 81 & 161 & 0.6 & \xmark & \xmark & & \\
        T & 101 & 101 & 0.6 & \cmark & \cmark & & \\
        T & 81 & 161 & 0.6 & \cmark & \cmark & 6.4 & 16.97 \\  %
        \midrule
        TF & 81 & 161 & 0.6 & \cmark & \cmark & 14.69 & 8.72 \\  %
        TF & 81 & 141 & 0.6 & \cmark & \cmark & 11.77 & 9.07 \\  %
        TF & 81 & 121 & 0.6 & \cmark & \cmark & 9.26 & 9.64 \\  %
        TF & 81 & 101 & 0.6 & \cmark & \cmark & 7.86 & 10.83 \\  %
        TF & 81 & 81 & 0.6 & \cmark & \cmark & 8.99 & 15.51 \\  %
        \midrule
        TF & 81 & 81 & 0.6 & \cmark & \cmark & 8.99 & 15.51 \\  %
        TF & 81 & 81 & 0.3 & \cmark & \cmark & 5.4 & 11.37 \\  %
        TF & 81 & 81 & 0.1 & \cmark & \cmark & 5.44 & 9.84 \\  %
        \midrule
        TF & 101 & 101 & 0.6 & \cmark & \cmark & 8.38 & 14.99 \\  %
        TF & 101 & 101 & 0.3 & \cmark & \cmark & 5.34 & 11.33 \\  %
        TF & 101 & 101 & 0.1 & \cmark & \cmark & \bf 5.52 & 9.83 \\  %
        \midrule
        TF & 81 & 161 & 0.6 & \cmark & \cmark & 14.69 & 8.72 \\  %
        TF & 81 & 161 & 0.3 & \cmark & \cmark & 16.28 & \bf 8.05 \\  %
        TF & 81 & 161 & 0.1 & \cmark & \cmark & 18.62 & 8.25 \\  %
    \bottomrule
  \end{tabular}
  
\end{table*}

